Efficient Emulation of Computer Models Utilising Multiple Known Boundaries of Differing Dimensions

Emulation has been successfully applied across a wide variety of scientific disciplines for efficiently analysing computationally intensive models. We develop known boundary emulation strategies which utilise the fact that, for many computer models, there exist hyperplanes in the input parameter space for which the model output can be evaluated far more efficiently, whether this be analytically or just significantly faster using a more efficient and simpler numerical solver. The information contained on these known hyperplanes, or boundaries, can be incorporated into the emulation process via analytical update, thus involving no additional computational cost. In this article, we show that such analytical updates are available for multiple boundaries of various dimensions. We subsequently demonstrate which configurations of boundaries such analytical updates are available for, in particular by presenting a set of conditions that such a set of boundaries must satisfy. We demonstrate the powerful computational advantages of the known boundary emulation techniques developed on both an illustrative low-dimensional simulated example and a scientifically relevant and high-dimensional systems biology model of hormonal crosstalk in the roots of an Arabidopsis plant.

==> ArXiv Version 13.03.20/Commands.tex <==
\newcommand{\BE}[2]{\text{E}_{#1}{[#2]}}
\newcommand{\BV}[2]{\text{Var}_{#1}{[#2]}}
\newcommand{\BC}[3]{\text{Cov}_{#1}{[#2},{#3}]}
\newcommand{\e}[1]{\ensuremath{{\rm E}[#1]}}
\newcommand{\ed}[2]{\ensuremath{{\rm E}_{#1}[#2]}}
\newcommand{\var}[1]{\ensuremath{{\rm Var}[#1]}}
\newcommand{\vard}[2]{\ensuremath{{\rm Var}_{#1}[#2]}}
\newcommand{\corr}[2]{\ensuremath{{\rm Corr}\left[#1,#2\right]}}
\newcommand{\corrd}[3]{\ensuremath{{\rm Corr}_{#1}\left[#2,#3\right]}}
\newcommand{\cov}[2]{\ensuremath{{\rm Cov}\left[#1,#2\right]}}
\newcommand{\covd}[3]{\ensuremath{{\rm Cov}_{#1}\left[#2,#3\right]}}

\newcommand{\covb}[2]{\ensuremath{{\rm Cov}[#1,#2]}}
\newcommand{\re}[2]{\ensuremath{{\rm r}_{#1}(#2)}\,}
\newcommand{\R}[3]{\ensuremath{{ R}_{#1}(#2,#3)}\,}
\newcommand{\RS}[4]{\ensuremath{{ R^{(2)}}_{#1}(#2,#3,#4)}}
\newcommand{\rvard}[2]{\ensuremath{{\rm RVar}_{#1}[#2]}}

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bn}{\begin{enumerate}}
\newcommand{\en}{\end{enumerate}}
\newcommand{\bfi}{\begin{figure}}
\newcommand{\efi}{\end{figure}}

\newcommand{\cm}[1]{\ensuremath{ { #1 }}}

\newcommand{\mx}{\mathcal{X}}
\newcommand{\mk}{\mathcal{K}}
\newcommand{\ml}{\mathcal{L}}
\newcommand{\mm}{\mathcal{M}}

\newcommand{\qq}{\quad \quad}

\newcommand{\ian}[1]{\textcolor{black}{#1}}% IRV comments/changes		
\newcommand{\sam}[1]{\textcolor{blue}{#1}}% JP comments/changes	

\newcommand{\iv}[1]{\textcolor{black}{#1}}% IRV comments/changes		
\newcommand{\ivm}[1]{\textcolor{black}{#1}}% IRV comments/changes		

% sequences
\newcommand{\seq}[2]{#1,\dots,#2}
\newcommand{\seqsub}[3]{\seq{#1_{#2}}{#1_{#3}}}
\newcommand{\seqsup}[3]{\seq{#1^{#2}}{#1^{#3}}}
\newcommand{\seqsupb}[3]{\seqsup{#1}{(#2)}{(#3)}}
\newcommand{\seqsupbf}[3]{\seq{f(#1^{(#2)})}{f(#1^{(#3)})}}

% shortest distance expression a^K = x - x^K
\newcommand{\shortdist}[1]{$ a^{#1} = x - x^{#1} $}

% covariance expressions
\newcommand{\covxB}[1]{\covb{f(x)}{f(x^{#1})}}
\newcommand{\covB}[1]{\covb{f(x)}{#1}}
\newcommand{\covDxB}[2]{\covd{#2}{f(x)}{f(x^#1)}}
\newcommand{\covDB}[2]{\covd{#2}{f(x)}{#1}}
\newcommand{\covDff}[3]{\covd{#1}{f(#2)}{f(#3)}}

% expectation expressions
\newcommand{\ef}[2]{\ed{#1}{f(#2)}}

% r functions
\newcommand{\rx}[3]{\re{#1}{#2-#3}}
\newcommand{\rxB}[2]{\rx{#1}{x}{x^#2}}
\newcommand{\ra}[1]{\re{J_#1}{a^#1}}
\newcommand{\raK}{\ra{K}}
\newcommand{\raL}{\ra{L}}
\newcommand{\rap}[1]{\re{J_#1}{a'^#1}}
\newcommand{\rapK}{\rap{K}}
\newcommand{\rapL}{\rap{L}}
\newcommand{\rp}[1]{\rx{P^{#1}}{x}{x'}}
\newcommand{\rxx}[1]{\re{J_{#1}}{x^#1-x'^#1}}
\newcommand{\raa}[1]{\re{J_{#1}}{a^#1-a'^#1}}
\newcommand{\rara}[1]{\re{J_{#1}}{a^{#1}}  \re{J_{#1}}{a'^{#1}}}
\newcommand{\raaK}{\raa{K}}

% R functions
\newcommand{\Ra}[1]{\R{J_#1}{a^#1}{a'^#1}}
\newcommand{\RaK}{\Ra{K}}

% ys and zs
\newcommand{\ys}{y^{(s)}}
\newcommand{\zs}{z^{(s)}}
\newcommand{\zsK}{z^{(s)K}}

% x^boundary
\newcommand{\xK}{x^K}
\newcommand{\xL}{x^L}
\newcommand{\xKL}{x^{KL}}
\newcommand{\xLK}{x^{LK}}
\newcommand{\aK}{a^K}
\newcommand{\aL}{a^L}
\newcommand{\aKL}{a^{KL}}
\newcommand{\aLK}{a^{LK}}
\newcommand{\xpK}{x'^K}
\newcommand{\xpL}{x'^L}
\newcommand{\xpKL}{x'^{KL}}
\newcommand{\xpLK}{x'^{LK}}
\newcommand{\apK}{a'^K}
\newcommand{\apL}{a'^L}
\newcommand{\apKL}{a'^{KL}}
\newcommand{\apLK}{a'^{LK}}
\newcommand{\akH}{a^{K_H}}
\newcommand{\apkH}{a'^{K_H}}
\newcommand{\akHm}{a^{K_{H-1}}}
\newcommand{\apkHm}{a'^{K_{H-1}}}
\newcommand{\akT}{a^{K_T}}
\newcommand{\apkT}{a'^{K_T}}


% trick
\newcommand{\trick}[1]{\cov{f(x^{#1})}{#1} \var{#1}^{-1} =\; (1,0, \cdots, 0)}
\newcommand{\trickD}[2]{\covd{#1}{f(x^{#2})}{#2} \vard{#1}{#2}^{-1} =\; (1,0, \cdots, 0)}

% generic commands
\newcommand{\butnot}{\backslash}
\newcommand{\sds}{\sigma^2 \,}
\newcommand{\capdots}{\cap \cdots \cap}
\newcommand{\cupdots}{\cup \cdots \cup}
\newcommand{\AEq}{\nonumber \\ & = &}
\newcommand{\AEqN}{\\ & = &}
\newcommand{\NL}{\nonumber \\ & & \qq }
\newcommand{\Df}[1]{\Delta f(#1)}
\newcommand{\tim}{\; \times \;}

% commands for Two perpendicular boundaries section
\newcommand{\Rxz}[2]{\R{J_{#1}}{x^{#2}-x^{#2#1}}{\zs - z^{(s)#1}}}
\newcommand{\rpxz}[2]{\rx{P^{#1}}{x^{#2}}{\zs}}
\newcommand{\rpKLxL}{\rpxz{K \cup L}{L}}
\newcommand{\rpKL}{\rpxz{K \cup L}{}}
\newcommand{\rpKaL}{\rp{K \cap L}}
\newcommand{\rpKoL}{\rp{K \cup L}}
\newcommand{\rLnK}[1]{\re{J_L \butnot J_K}{#1}}
\newcommand{\rKnL}[1]{\re{J_K \butnot J_L}{#1}}
\newcommand{\rKL}[1]{\re{J_K \cap J_L}{#1}}
\newcommand{\rKoL}[1]{\re{J_K \cup J_L}{#1}}
\newcommand{\rK}[1]{\re{J_K}{#1}}
\newcommand{\rL}[1]{\re{J_L}{#1}}
\newcommand{\RK}[2]{\R{J_K}{#1}{#2}}
\newcommand{\RL}[2]{\R{J_L}{#1}{#2}}
\newcommand{\RLnK}[2]{\R{J_L \butnot J_K}{#1}{#2}}
\newcommand{\RKnL}[2]{\R{J_K \butnot J_L}{#1}{#2}}
\newcommand{\RKL}[2]{\R{J_K \cap J_L}{#1}{#2}}
\newcommand{\RKoL}[2]{\R{J_K \cup J_L}{#1}{#2}}
\newcommand{\xKh}{x^{K_h}}
\newcommand{\xpKh}{x'^{K_h}}
\newcommand{\aKh}{a^{K_h}}
\newcommand{\apKh}{a'^{K_h}}

% commands for Multiple perpendicular boundaries section
\newcommand{\mkH}{\mk_H}
\newcommand{\KH}{K_H}
\newcommand{\KHm}{K_{H-1}}
\newcommand{\rKT}{\re{J_T}{a^{K_T}}}
\newcommand{\RH}{\R{{\KH}}{x}{x'}}
\newcommand{\RHm}{\R{{\KHm}}{x}{x'}}
\newcommand{\rT}[1]{\re{J_T}{#1}}
\newcommand{\rH}[1]{\re{J_H}{#1}}
\newcommand{\rHnT}[1]{\re{J_H \butnot J_T}{#1}}
\newcommand{\rHmnT}[1]{\re{J_{H-1} \butnot J_T}{#1}}
\newcommand{\rpH}[1]{\re{P^H}{#1}}
\newcommand{\rpHm}[1]{\re{P^{H-1}}{#1}}
\newcommand{\zsKHm}{z^{(s)K_{H-1}}}
\newcommand{\xKhKHm}{x^{K_hK_{H-1}}}
\newcommand{\xpKhKHm}{x'^{K_hK_{H-1}}}
\newcommand{\rTnh}[1]{\re{J_T \butnot J_h}{#1}}
\newcommand{\rTh}[1]{\re{J_T \cap J_h}{#1}}
\newcommand{\rHmh}[1]{\re{J_{H-1} \cap J_h}{#1}}
\newcommand{\xKHm}{x^{K_{H-1}}}
\newcommand{\rh}[1]{\re{J_h}{#1}}
\newcommand{\xKhKT}{x^{K_hK_T}}
\newcommand{\xKT}{x^{K_T}}
\newcommand{\aKhKT}{a^{K_hK_T}}

% commands for Multiple parallel boundaries section
\newcommand{\Rg}[4]{\ensuremath{{ R}^{(#1)}_{#2}(#3,#4)}\,}
\newcommand{\gmm}{\gamma - 1}
\newcommand{\Kg}{K_\gamma}
\newcommand{\KG}{K_\Gamma}
\newcommand{\KGm}{K_{\Gamma - 1}}
\newcommand{\KgKGm}{\Kg\KGm}
\newcommand{\rgnGm}[1]{\re{J_\gamma \butnot J_{\Gamma - 1}}{#1}}
\newcommand{\aKg}{a^{K_\gamma}}
\newcommand{\apKg}{a'^{K_\gamma}}
\newcommand{\xKg}{x^{K_\gamma}}
\newcommand{\sumig}{\sum_{i=2}^\gamma}
\newcommand{\sumbG}{\sum_{b \subset \Gamma, \, b_1 < ... < b_i = \gamma}}
\newcommand{\sumihm}{\sum_{i=1}^{h-1}}
\newcommand{\sumihz}{\sum_{i=0}^{h-1}}
\newcommand{\sumTHm}{\sum_{T \subseteq H_{-1}, \, |T| = i}}
\newcommand{\sumTH}{\sum_{T \subseteq H, |T| = i}}
\newcommand{\prodli}{\prod_{l=1}^{i-1}}
\newcommand{\blm}{b_l - 1}
\newcommand{\KBlm}{K_{B_l - 1}}
\newcommand{\Kbl}{K_{b_l}}
\newcommand{\KgKBlm}{\Kg \KBlm}
\newcommand{\KblKBlm}{\Kbl \KBlm}
\newcommand{\rblnBlm}[1]{\re{J_{b_l} \butnot J_{B_l - 1}}{#1}}
\newcommand{\Kblp}{K_{b_{l+1}}}
\newcommand{\xKb}{x^{K_b}}
\newcommand{\rHmnToh}[1]{\re{J_{H-1} \butnot (J_T \cup J_h)}{#1}}
\newcommand{\rhnHm}[1]{\re{J_h \butnot J_{H-1}}{#1}}
\newcommand{\rHmhnT}[1]{\re{(J_{H-1} \cap J_h) \butnot J_T}{#1}}
\newcommand{\rHmohnT}[1]{\re{(J_{H-1} \cup J_h) \butnot J_T}{#1}}
\newcommand{\rToh}[1]{\re{J_T \cup J_h}{#1}}
\newcommand{\aKTKh}{a^{K_TK_h}}

% commands for 3D example
\newcommand{\ro}[1]{\re{1}{#1}}
\newcommand{\rtt}[1]{\re{\{2,3\}}{#1}}
\newcommand{\Rtt}[2]{\R{\{2,3\}}{#1}{#2}}
\newcommand{\aM}{a^M}
\newcommand{\xM}{x^M}

\newcommand{\ifelsearray}[4]{\left\{ \begin{array}{r@{\quad \mbox{if} \quad}l} #1 & #2 \\ #3 & #4  \end{array} \right.}

==> ArXiv Version 13.03.20/Definitions.tex <==
\def \simulator { f }
\def \simulatorx { f(x) }
\def \simulatorX { f(X) }
\def \simulatorruns { \{ f(x^{(1)}),...,f(x^{(n)}) \} }
\def \regcomp { \sum_{j=1}^{m_i} \beta_{ij} g_{ij}(x) }
\def \rescomp { u_i(x) }
\def \nugget { \omega(x) }
\def \expectation  {\textrm{E}} 
\def \variance {\textrm{Var} }
\def \covariance {\textrm{Cov} }
\def \correlation {\textrm{Corr} }
\def \fbexp { \mathbb{E} }
\def \fbvar { \mathbb{V}ar }
\def \fbcov { \mathbb{C}ov }
\def \optindV { i^{(1)}, ..., i^{(n)} }
\def \optindU { i^{(n+1)}, ..., i^{(n+m)} }
\def \designset { X_D}
\def \Xv { x^{(1)}, ..., x^{(n)} }
\def \Xu { x^{(n+1)}, ..., x^{(n+m)} }
\def \FXv { \{ \simulator_{i^{(1)}}(x^{(1)}), ..., \simulator_{i^{(n)}}(x^{(n)}) \} }
\def \FXu { \{ \simulator_{i_B^{(1)}}(x_B^{(1)}), ..., \simulator_{i_B^{(n_B)}}(x^{(n_B)}) \} }
\def \Sig { \mathbf{\Sigma} }
\def \mean { \mu }
\def \dist { \pi }
\def \para { \tau }
\def \cl { \theta }
\def \actinp { A_i }
\def \corrmat {C}
\def \Simulator { F(x) }
\def \Regfun { G }
\def \regfunx { g(x) }
\def \indicator { \mathbb{I} }
\def \obs { z }
\def \md { \epsilon }
\def \me { e }
\def \system { y }
\def \independent {\perp\!\!\!\perp} 
\def \mevar { \sigma^2_{\me} }
\def \mdvar { \sigma^2_{\md} }
\def \mcvar { \sigma^2_c }
\def \mevari { \sigma^2_{\me_i} }
\def \mdvari { \sigma^2_{\md_i} }
\def \mcvari { \sigma^2_{c_i} }
\def \bestx { x^\star }
\def \Bestx {X^\star}
\def \simbestx { \simulator(\bestx) }
\def \imp { I }
\def \setx { \mathcal{X} }
\def \bestset { \setx^\star }
\def \sigmd { \Sig_{\md} }
\def \sigme { \Sig_{\me} }
\def \rv { W }
\def \DS { G }
\def \indimp { \mathcal{I} }
\def \SCO { \mathcal{S} }
\def \vol { V }
\def \Obs { Z }
\def \GP { \mathcal{GP} }
\def \normal { \mathcal{N} }
\def \nsx { n_c }
\def \nsz { n_{sim} }
\def \nchoo {n}
\def \nup {u}
\def \nexp {N}
\def \expset {d}
\def \mevara { \sigma^2_{\me, \expset} }
\def \mdvara { \sigma^2_{\md, \expset} }
\def \oc { r }
\def \ocset { \mathcal{R} }
\def \gam { \rho }
\def \gamset { \mathcal{P} }
\def \uf { u }
\def \real { \mathbb{R} }
\def \pref { \preceq }
\def \dec { d }
\def \Dec { \mathcal{D} }
\def \bestdec { d^\star }
\def \rq { w }
\def \RQ { \mathcal{W} }
\def \posexpset { \mathcal{Y}_f }
\def \posexp { y }
\def \tf { g }
\def \weight { \omega }
\def \vf { v }
\def \res { R }
\def \detvar { Q }
\def \optres { T }
\def \geninv { \dagger }
\def \cost { \mathcal{C} }
\def \maxcost { C^{m} }
\def \rawobs { \phi }
\def \Rawobs { \Phi }
\def \pf { \eta }
\def \xc { x^C }
\def \xe { x^E }
\def \xm { x^M }
\def \Xc { X^C }
\def \Xe { X^E }
\def \Xm { X^M }
\def \xcset { \hat{X}^C }
\def \dose { \Gamma }
\def \trace { Tr }
\def \nsim { n_{D} }
\def \nsimo { n_{D_o} }
\def \nsimn { n_{D^\prime} }
\def \ndes { m_D }
\def \nsimDp { m_{D^\prime} }
\def \dim { d }
\def \dessimset { \Psi }
\def \dessim { \psi }
\def \desxset { \Xi }
\def \desx { \xi }
\def \det {\textrm {det}}
\def \trace {\textrm {trace}}
\def \recrate { \gamma }
\def \infrate { \beta }
